Public-Key Encryption from the MinRank Problem

We construct a public-key encryption scheme from the hardness of the (planted) MinRank problem over uniformly random instances. This corresponds to the hardness of decoding random linear rank-metric codes. Existing constructions of public-key encryption from such problems require hardness for structured instances arising from the masking of efficiently decodable codes. Central to our construction is the development of a new notion of duality for rank-metric codes.

==> lncs_issues.tex <==
%!TEX root = main.tex

%% Fixes to lncs class

\makeatletter
\def\@thmcountersep{.}
\def\@thmcounterend{.}

\def\spnewtheorem{\@ifstar{\@sthm}{\@Sthm}}

% definition of \spnewtheorem with number

\def\@spnthm#1#2{%
	\@ifnextchar[{\@spxnthm{#1}{#2}}{\@spynthm{#1}{#2}}}
\def\@Sthm#1{\@ifnextchar[{\@spothm{#1}}{\@spnthm{#1}}}

\def\@spxnthm#1#2[#3]#4#5{\expandafter\@ifdefinable\csname #1\endcsname
	{\@definecounter{#1}\@addtoreset{#1}{#3}%
		\expandafter\xdef\csname the#1\endcsname{\expandafter\noexpand
			\csname the#3\endcsname \noexpand\@thmcountersep \@thmcounter{#1}}%
		\expandafter\xdef\csname #1name\endcsname{#2}%
		\global\@namedef{#1}{\@spthm{#1}{\csname #1name\endcsname}{#4}{#5}}%
		\global\@namedef{end#1}{\@endtheorem}}}

\def\@spynthm#1#2#3#4{\expandafter\@ifdefinable\csname #1\endcsname
	{\@definecounter{#1}%
		\expandafter\xdef\csname the#1\endcsname{\@thmcounter{#1}}%
		\expandafter\xdef\csname #1name\endcsname{#2}%
		\global\@namedef{#1}{\@spthm{#1}{\csname #1name\endcsname}{#3}{#4}}%
		\global\@namedef{end#1}{\@endtheorem}}}

\def\@spothm#1[#2]#3#4#5{%
	\@ifundefined{c@#2}{\@latexerr{No theorem environment `#2' defined}\@eha}%
	{\expandafter\@ifdefinable\csname #1\endcsname
		{\newaliascnt{#1}{#2}%
			\expandafter\xdef\csname #1name\endcsname{#3}%
			\global\@namedef{#1}{\@spthm{#1}{\csname #1name\endcsname}{#4}{#5}}%
			\global\@namedef{end#1}{\@endtheorem}}}}

\def\@spthm#1#2#3#4{\topsep 7\p@ \@plus2\p@ \@minus4\p@
	\refstepcounter{#1}%
	\@ifnextchar[{\@spythm{#1}{#2}{#3}{#4}}{\@spxthm{#1}{#2}{#3}{#4}}}

\def\@spxthm#1#2#3#4{\@spbegintheorem{#2}{\csname the#1\endcsname}{#3}{#4}%
	\ignorespaces}

\def\@spythm#1#2#3#4[#5]{\@spopargbegintheorem{#2}{\csname
		the#1\endcsname}{#5}{#3}{#4}\ignorespaces}

\def\@spbegintheorem#1#2#3#4{\trivlist
	\item[\hskip\labelsep{#3#1\ #2\@thmcounterend}]#4}

\def\@spopargbegintheorem#1#2#3#4#5{\trivlist
	\item[\hskip\labelsep{#4#1\ #2}]{#4(#3)\@thmcounterend\ }#5}

% definition of \spnewtheorem* without number

\def\@sthm#1#2{\@Ynthm{#1}{#2}}

\def\@Ynthm#1#2#3#4{\expandafter\@ifdefinable\csname #1\endcsname
	{\global\@namedef{#1}{\@Thm{\csname #1name\endcsname}{#3}{#4}}%
		\expandafter\xdef\csname #1name\endcsname{#2}%
		\global\@namedef{end#1}{\@endtheorem}}}

\def\@Thm#1#2#3{\topsep 7\p@ \@plus2\p@ \@minus4\p@
	\@ifnextchar[{\@Ythm{#1}{#2}{#3}}{\@Xthm{#1}{#2}{#3}}}

\def\@Xthm#1#2#3{\@Begintheorem{#1}{#2}{#3}\ignorespaces}

\def\@Ythm#1#2#3[#4]{\@Opargbegintheorem{#1}
	{#4}{#2}{#3}\ignorespaces}

\def\@Begintheorem#1#2#3{#3\trivlist
	\item[\hskip\labelsep{#2#1\@thmcounterend}]}

\def\@Opargbegintheorem#1#2#3#4{#4\trivlist
	\item[\hskip\labelsep{#3#1}]{#3(#2)\@thmcounterend\ }}

%\if@envcntsect
%\def\@thmcountersep{.}
%\spnewtheorem{theorem}{Theorem}[section]{\bfseries}{\itshape}
%\else
%\spnewtheorem{theorem}{Theorem}{\bfseries}{\itshape}
%\if@envcntreset
%\@addtoreset{theorem}{section}
%\else
%\@addtoreset{theorem}{chapter}
%\fi
%\fi

%definition of divers theorem environments
\if@envcntsame % alle Umgebungen wie Theorem.
\def\spn@wtheorem#1#2#3#4{\@spothm{#1}[theorem]{#2}{#3}{#4}}
\else % alle Umgebungen mit eigenem Zaehler
\if@envcntsect % mit section numeriert
\def\spn@wtheorem#1#2#3#4{\@spxnthm{#1}{#2}[section]{#3}{#4}}
\else % nicht mit section numeriert
\if@envcntreset
\def\spn@wtheorem#1#2#3#4{\@spynthm{#1}{#2}{#3}{#4}
	\@addtoreset{#1}{section}}
\else
\def\spn@wtheorem#1#2#3#4{\@spynthm{#1}{#2}{#3}{#4}
	\@addtoreset{#1}{chapter}}%
\fi
\fi
\fi


% \spn@wtheorem{fact}{Fact}{\bfseries}{\itshape}
% \spn@wtheorem{assumption}{Assumption}{\bfseries}{\itshape}
% \spn@wtheorem{myclaim}{Claim}{\bfseries}{\itshape}
% \Crefname{myclaim}{Claim}{Claims}
% \makeatother
